Empowering Citizens by a Blockchain-Based Robinson List

A Robinson list protects phone subscribers against commercial spam calls. Its least basic functionality is to collect the denial of the subscribers to be contacted by market operators. Nowadays, Robinson lists run as centralised services, which implies that citizens should trust third parties for the management of their choices. In this paper, we show a design that allows us to realise a Robinson list as a decentralised service. Our work leverages the experience developed by Fondazione Ugo Bordoni as the manager of the Italian Robinson list. We present a general solution and a proof-of-concept (PoC) adopting the Algorand technology. We evaluate the performances of our PoC in terms of its scalability and of the latency perceived by the involved actors. We also discuss aspects related to identity management and privacy.

==> discussion.tex <==


\begin{comment}
\section{Discussion}\label{sec:discussion}

\todo[inline]{how requirements are met.
I todo seguenti sono stati portati qui dal fondo di solution dove è stato messo un reference}

\todo[inline]{inserire qui qualche commento sulla sicurezza? o mettere in discussion?}

\todo[inline]{Queste considerazioni vanno messe qui in fondo o in discussion. vincoli e possibilità del initializer rispetto agli assets?
	Può creare nuovi asset dopo? forse si ma irrilevante per la sicurezza.
	
	può trasferirli al telephon number in violazione del option constraint? no perché $U_t$ accetta solo 
	transazioni firmate da $t$.
	
	può riprenderseli effettuando un DoS? Non dovrebbe.}

\end{comment}
